The Emergence of Bulges and Disks in the Universe

This thesis makes use of the imaging data from the Advanced Camera for Surveys (ACS) of the Hubble Space Telescope (HST) in the Cosmic Evolution Survey (COSMOS) and the Deep Extragalactic VIsible Legacy Survey (DEVILS) field. We provide visual morphological classifications of 44,000 galaxies out to redshift $z = 1$ and above a stellar mass of $10^{9.5} M_\odot$ (D10/ACS sample). We perform a robust Bayesian bulge-disk decomposition analysis of the D10/ACS sample. This study forms one of the largest morphological classification and structural analyses catalogues in this field to date. Using these catalogues, we explore the evolution of the stellar mass function (SMF) and the stellar mass density (SMD) together with the stellar mass-size relations ($M_*-R_e$) of galaxies as a function of morphological type as well as for disks and bulges, separately. We quantify that one-third of the current stellar mass of the Universe was formed during the last 8 Gyr. We find that the moderate growth of the high-mass end of the SMF is dominated by the growth of elliptical systems and that the vast majority of the stellar mass of the Universe is locked up in disk+bulge systems at all epochs and that they increase their contribution to the total SMD with time. The contribution of the pure-disk morphology gradually decreases with time ($\sim40\%$), while ellipticals increase their contribution by a factor of $1.7$ since $z = 1$. By decomposing galaxies into disks and bulges we quantify that on average $\sim50\%$ of the total stellar mass of the Universe at all epochs is in disk structures with this contribution relatively unchanged since $z \sim 0.6$. With this comes more rapid growth of pseudo-bulges and spheroids (bulges and ellipticals) in mass. Furthermore, while the cosmic star-formation history is declining the Universe is transitioning from a disk dominated era to ...

==> proofs/dups <==
#!/usr/bin/env perl

# Finds duplicate adjacent words.

use strict ;

my $DupCount = 0 ;

if (!@ARGV) {
  print "usage: dups <file> ...\n" ;
  exit ;
}

while (1) {
  my $FileName = shift @ARGV ;

# Exit code = number of duplicates found.
  exit $DupCount if (!$FileName) ;

  open FILE, $FileName or die $!;

  my $LastWord = "" ;
  my $LineNum = 0 ;

  while (<FILE>) {
    chomp ;

    $LineNum ++ ;

    my @words = split (/(\W+)/) ;

    foreach my $word (@words) {
# Skip spaces:
      next if $word =~ /^\s*$/ ;

# Skip punctuation:
      if ($word =~ /^\W+$/) {
        $LastWord = "" ;
        next ;
      }

# Found a dup?
      if (lc($word) eq lc($LastWord)) {
        print "$FileName:$LineNum $word\n" ;
        $DupCount ++ ;
      } # Thanks to Sean Cronin for tip on case.

# Mark this as the last word:
      $LastWord = $word ;
    }
  }

  close FILE ;
}


==> proofs/passive <==
#!/bin/bash

irregulars="awoken|\
            been|born|beat|\
            become|begun|bent|\
            beset|bet|bid|\
            bidden|bound|bitten|\
            bled|blown|broken|\
            bred|brought|broadcast|\
            built|burnt|burst|\
            bought|cast|caught|\
            chosen|clung|come|\
            cost|crept|cut|\
            dealt|dug|dived|\
            done|drawn|dreamt|\
            driven|drunk|eaten|fallen|\
            fed|felt|fought|found|\
            fit|fled|flung|flown|\
            forbidden|forgotten|\
            foregone|forgiven|\
            forsaken|frozen|\
            gotten|given|gone|\
            ground|grown|hung|\
            heard|hidden|hit|\
            held|hurt|kept|knelt|\
            knit|known|laid|led|\
            leapt|learnt|left|\
            lent|let|lain|lighted|\
            lost|made|meant|met|\
            misspelt|mistaken|mown|\
            overcome|overdone|overtaken|\
            overthrown|paid|pled|proven|\
            put|quit|read|rid|ridden|\
            rung|risen|run|sawn|said|\
            seen|sought|sold|sent|\
            set|sewn|shaken|shaven|\
            shorn|shed|shone|shod|\
            shot|shown|shrunk|shut|\
            sung|sunk|sat|slept|\
            slain|slid|slung|slit|\
            smitten|sown|spoken|sped|\
            spent|spilt|spun|spit|\
            split|spread|sprung|stood|\
            stolen|stuck|stung|stunk|\
            stridden|struck|strung|\
            striven|sworn|swept|\
            swollen|swum|swung|taken|\
            taught|torn|told|thought|\
            thrived|thrown|thrust|\
            trodden|understood|upheld|\
            upset|woken|worn|woven|\
            wed|wept|wound|won|\
            withheld|withstood|wrung|\
            written"

 if [ "$1" = "" ]; then
   echo "usage: `basename $0` <file> ..."
   exit
 fi

 egrep -n -i --color "\\b(am|are|were|being|is|been|was|be)\\b[ ]*(\w+ed|($irregulars))\\b" $*

exit $?


==> proofs/weasel <==
#!/bin/bash

weasels="many|various|very|fairly|several|extremely\
         |exceedingly|quite|remarkably|few|surprisingly\
         |mostly|largely|huge|tiny|((are|is) a number)\
         |excellent|interestingly|significantly\
         |substantially|clearly|vast|relatively|completely"

         wordfile=""

# Check for an alternate weasel file
         if [ -f $HOME/etc/words/weasels ]; then
         wordfile="$HOME/etc/words/weasels"
         fi

         if [ -f $WORDSDIR/weasels ]; then
         wordfile="$WORDSDIR/weasels"
         fi

         if [ -f words/weasels ]; then
         wordfile="words/weasels"
         fi

         if [ ! "$wordfile" = "" ]; then
         weasels="xyzabc123";
         for w in `cat $wordfile`; do
         weasels="$weasels|$w"
         done
         fi


         if [ "$1" = "" ]; then
         echo "usage: `basename $0` <file> ..."
         exit
         fi

         egrep -i -n --color "\\b($weasels)\\b" $*

         exit $?

